Security Advice for Parents and Children About Content Filtering and Circumvention as Found on YouTube and TikTok

In today's digital age, concerns about online security and privacy have become paramount. However, addressing these issues can be difficult, especially within the context of family relationships, wherein parents and children may have conflicting interests. In this environment, parents and children may turn to online security advice to determine how to proceed. In this paper, we examine the advice available to parents and children regarding content filtering and circumvention as found on YouTube and TikTok. In an analysis of 839 videos returned from queries on these topics, we found that half (n=399) provide relevant advice. Our results show that of these videos, roughly three-quarters are accurate, with the remaining one-fourth containing factually incorrect advice. We find that videos targeting children are both more likely to be incorrect and actionable than videos targeting parents, leaving children at increased risk of taking harmful action. Moreover, we find that while advice videos targeting parents will occasionally discuss the ethics of content filtering and device monitoring (including recommendations to respect children's autonomy) no such discussion of the ethics or risks of circumventing content filtering is given to children, leaving them unaware of any risks that may be involved with doing so. Ultimately, our research indicates that video-based social media sites are already effective sources of security advice propagation and that the public would benefit from security researchers and practitioners engaging more with these platforms, both for the creation of content and of tools designed to help with more effective filtering.

==> appx_queries.tex <==
\section{Search Queries}
\label{appx:queries}

\subsection{Parent queries}

\textbf{Initial queries:} \\
How to protect my child online \\
How to secure the Internet \\
How to block social media \\
How to block inappropriate content \\
How to block porn \\
How to stop kids from chatting with strangers online \\
How to protect kids in online gaming \\
How to disconnect devices at night \\
How to disconnect devices at dinner \\
How to setup OpenVPN \\

\noindent\textbf{Supplemental queries:} \\
How to set up DNS filters \\
How to set up content filters \\
How to limit social media time \\
How to see hidden apps on phone \\
Is my internet secure \\
Should I limit my kids internet \\
Should I monitor my kids online

\subsection{Child queries}
How do I unblock my device from the wifi \\
How do I access TikTok past bedtime \\
How do I access Instagram past bedtime \\
How do I access Facebook past bedtime \\
How do I keep my parents from monitoring my phone \\
How do I get around internet filters \\
How do I access TikTok on school wifi \\
How do I access Instagram on school wifi \\
How do I access Facebook on school wifi \\
How do I use a VPN \\
How can I access my neighbor’s wifi \\
How can I keep my parents from restricting what I watch \\
How can I unlock my school chromebook \\
How to get around screen time limits \\
How do I hide stuff on my phone from my parents \\
How do I hide apps on my phone

==> pilot.tex <==
\section{Exploratory Study}\label{pilot}

We began our investigation by looking into videos on TikTok and YouTube on the subject of DNS-based content filtering.
In this effort, we gathered and evaluated 230 videos between September 2022 and November 2022.
This study didn't need approval from our Institutional Review Board (IRB) because it involved only publicly available data and didn't involve any interventions with human subjects.

The purpose of this exploratory study was two-fold.
First, we wanted to get a better sense of the topics being discussed around content filtering and determine whether DNS-based content filtering was too narrow a scope (it was).
Second, we wanted to build a code book that could be used to describe the videos we watched.
Ultimately, the results of this exploratory study were used to inform the design and execution of our full study (described in the next Section).

\subsection{Video Collection}
Two researchers manually searched for videos discussing DNS-based content filtering on YouTube and TikTok.
These researchers focused on videos targeted at (i) helping parents set up content filtering, (ii) helping children circumvent content filtering, and (iii) helping parents stop children's circumvention efforts.
For the initial set of search queries, the researchers attempted to mimic queries they felt an average teenager or parents would use to learn about content filtering.
From the parent side, example search terms include, ``Setting up parental controls,'' ``Monitoring children's tech usage,'' ``How to block websites not suitable for kids,'' and ``Wi-Fi filters for children.''
For teenages, example search terms included ``get around internet filter,'' ``unblock Wi-Fi,'' and ``unblock school Chromebook.''

After collecting and viewing relevant videos returned by these initial queries, the researchers then created several follow-up queries that they felt users would search to fill in informational gaps from the initial queries.
Data collection continued in this manner until the researchers felt that they had reached saturation, which in this case we define as running 2 or 3 queries in which no new relevant videos or topics were identified.
Throughout the data collection process, the two researchers worked collaboratively, continuously gathering relevant video content. They also documented various aspects of the videos, including likes, views, and comments.

%For example, one video had around 1.5 million views, 18,000 likes, and 3,300 comments, which was on the high end.

\paragraph{Bias Control}
The two social media platforms we utilized are known for employing black-box algorithms to tailor content for their users. On TikTok, the 'For You Page' offers an endlessly scrolling feed of short videos, personalized for each user. Similarly, YouTube utilizes a comparable approach, suggesting content to users based on their viewing history and other factors.

To mitigate biases stemming from user-specific watch histories, we opted to create entirely new accounts on both platforms, with these accounts accessed from incognito browser sessions.
We also used separate accounts for the adult and child searches.
This approach helps ensure that any tailoring of the search results caused by the algorithms is confined to our prior searches, simulating the experience of a single user exploring content filtering.

\subsection{Video Analysis}

Three researchers (including the two researchers doing data collection) analyzed the collected videos using the first stages of the grounded theory methodology~\cite{strauss1997grounded}.
First, watching the videos together, the researchers performed open coding of the video's content examining video topics, motivations, and style.
Second, after open coding was finished, the coders used axial coding to group related codes into distinct concepts.
Based on these concepts and their interconnections, researchers grouped related concepts, generating themes, and describing how the concepts in the videos related to each other.
Most importantly, these concepts, themes, and their interconnections were used to craft the codebook used to evaluate videos in our full study.

\subsection{Results}

\begin{table*}
	\centering
	\begin{tabular}{ll|r|r|r|r}
		& Methodology & \multicolumn{1}{c|}{N} & \multicolumn{1}{c|}{\shortstack{Total\\Views}} & \multicolumn{1}{c|}{\shortstack{Total\\Likes}} & \multicolumn{1}{c}{\shortstack{Total\\Comments}} \\ \midrule 
		\multirow{4}{*}{Parents}
		& Parental control apps & 29 &  2,948,767 & 21,328 & 233  \\
		& Content filtering & 14 & 3,365,836 & 29,144  & 11 \\
		& Location tracking apps & 5 & 340,600  & 9,423  & 104 \\ \cmidrule{2-6}
		& Others & 67 & 2,563,580 & 3,650,480 & 305  \\ \midrule
		
		\multirow{6}{*}{Kids}
		& VPN & 23 & 1,862,352 & 45,586 & 3,775 \\
		& Changing network address &  19 & 114,186 & 37,165 & 6,666 \\
		& Proxy & 13 & 323,049 & 3,480 & 1109 \\
		& Alternate network & 9 & 4,000 & 423 & 76 \\
		& Device reset &  8 & 9,403 & 1,047 & 660 \\ \cmidrule{2-6}
		& Others &  43 & 4,835,753 & 1,130,115   &9,896  \\ \bottomrule 
	\end{tabular}
	\caption{Overview of video topics and metrics for the exploratory study}
	\label{tab:initial_study}
\end{table*}

In total, we collected a total of 229 videos from both YouTube and TikTok.
Of these, 115 focused on educating parents and guiding them in setting up parental controls, while the remaining 115 focused on techniques for bypassing restrictions.
Table~\ref{tab:initial_study} shows a summary of the most common topics along with their cumulative views, likes, and comments for each technique that is found either in the parents' or kids' context. 
In general, the videos had a wide range of engagement, from very few views and interactions to some with high popularity.

